LISA Dynamics & Control: Closed-loop Simulation and Numerical Demonstration of Time Delay Interferometry

The Laser Interferometer Space Antenna (LISA), space-based gravitational wave observatory involves a complex multidimensional closed-loop dynamical system. Its instrument performance is expected to be less efficiently isolated from platform motion than was its simpler technological demonstrator, LISA Pathfinder. It is of crucial importance to understand and model LISA dynamical behavior accurately to understand the propagation of dynamical excitations through the response of the instrument down to the interferometer data streams. More generally, simulation of the system allows for the preparation of the processing and interpretation of in-flight metrology data. In this work, we present a comprehensive mathematical modeling of the closed-loop system dynamics and its numerical implementation within the LISA Consortium simulation suite. We provide, for the first time, a full time-domain numerical demonstration of post-processing Time Delay Interferometer techniques combining multiple position measurements with realistic control loops to create a synthetic Michelson interferometer. We show that in the absence of physical coupling to spacecraft and telescope motion (through tilt-to-length, stiffness and actuation cross-talk) the effect of noisy spacecraft motion is efficiently suppressed to a level below the noise originating in the rest of the instrument.

==> commands.tex <==
\newcommand{\indice}[1]{{\scriptscriptstyle #1}}
\newcommand{\exposant}[1]{{\scriptscriptstyle #1}}
\newcommand{\myvec}[2]{\va*{#1}_\indice{#2}}
\newcommandx{\mylongvec}[4][2=,4=]{\vv{\mathbf{#1}_\indice{#2}\mathbf{#3}_\indice{#4}}}
\newcommand{\myexpr}[3]{#1_\indice{#2}^\exposant{#3}}
\newcommandx{\ddt}[3][3=]{ \dv{t}\Bigg|_\indice{\mathcal{#2}_{#3}} \mspace{-10mu} \left[ #1 \right]}
\newcommandx{\ddtddt}[3][3=]{ \dv[2]{t}\Bigg|_\indice{\mathcal{#2}_{#3}} \mspace{-10mu} \left[ #1 \right]}
\newcommand{\myhyperref}[1]{\hyperref[#1]{\ref{#1}}}
\newcommand{\identite}[1]{{\displaystyle \mathbb{1}_{\indice{#1}}}}
\newcommand{\myat}[2][]{#1|_{#2}}
\newcommand{\timestentothe}[1]{\times 10^{#1}}
\newcommand{\msout}[1]{\text{\sout{\ensuremath{#1}}}}

\newcommandx{\cardanvec}[4][2=,4=]{\myvec{\alpha}{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}
\newcommandx{\thetacardan}[4][2=,4=]{\theta_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}
\newcommandx{\etacardan}[4][2=,4=]{\eta_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}
\newcommandx{\phicardan}[4][2=,4=]{\phi_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}
\newcommandx{\cardanvecdot}[4][2=,4=]{\dv{\myvec{\alpha}{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}{t}}
\newcommandx{\thetacardandot}[4][2=,4=]{\dot{\theta}_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}
\newcommandx{\etacardandot}[4][2=,4=]{\dot{\eta}_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}
\newcommandx{\phicardandot}[4][2=,4=]{\dot{\phi}_\indice{{\mathcal{#1}_\indice{#2}/\mathcal{#3}_\indice{#4}}}}

\newcommandx{\vangvel}[6][2=,3=,5=,6=]{\myvec{\omega}{\mathcal{#1}_\indice{#2}^\exposant{#3}/\mathcal{#4}_\indice{#5}^\exposant{#6}}}

\newcommandx{\framevu}[3][3=]{\vu{e}_{#2,\mathcal{#1}_\indice{#3}}}
\newcommand{\framevus}[2]{\vu{e}_{#1_\indice{#2}}}

\newcommandx{\rotmat}[4][2=,4=]{\myexpr{T}{\mathcal{#3}_\indice{#4}}{\mathcal{#1}_\indice{#2}}}

\newcommand{\sint}[1]{s_{#1}}
\newcommand{\cost}[1]{c_{#1}}

\newcommandx{\posvec}[4][2=,4=]{\myvec{r}{#1_\indice{#2} / #3_\indice{#4}}}
\newcommandx{\velvec}[4][2=,4=]{\myvec{v}{#1_\indice{#2} / #3_\indice{#4}}}
\newcommandx{\posvecexp}[6][2=,4=,6=]{\myexpr{r}{#1_\indice{#2} / #3_\indice{#4}}{\mathcal{#5}_\indice{#6}}}
\newcommandx{\velvecexp}[6][2=,4=,6=]{\myexpr{\dot{r}}{#1_\indice{#2} / #3_\indice{#4}}{\mathcal{#5}_\indice{#6}}}
\newcommandx{\accvecexp}[6][2=,4=,6=]{\myexpr{\ddot{r}}{#1_\indice{#2} / #3_\indice{#4}}{\mathcal{#5}_\indice{#6}}}

\newcommandx{\vangvelexp}[6][2=,4=,6=]{\myexpr{\omega}{\mathcal{#1}_\indice{#2} / \mathcal{#3}_\indice{#4}}{\mathcal{#5}_\indice{#6}}}
\newcommandx{\vangaccexp}[6][2=,4=,6=]{\myexpr{\dot{\omega}}{\mathcal{#1}_\indice{#2} / \mathcal{#3}_\indice{#4}}{\mathcal{#5}_\indice{#6}}}

\newcommandx{\force}[4][2=,4=]{\myexpr{f}{#1_\indice{#2}}{\mathcal{#3}_\indice{#4}}}
\newcommandx{\torque}[4][2=,4=]{\myexpr{t}{#1_\indice{#2}}{\mathcal{#3}_\indice{#4}}}

\newcommand{\mytensor}[2]{\vb{#1}_\indice{#2}}
\newcommandx{\itensor}[3][3=]{\mytensor{I}{\text{#1}/#2_\indice{#3}}}
\newcommandx{\itensorexp}[5][3=,5=]{\myexpr{I}{\text{#1}/#2_\indice{#3}}{\mathcal{#4}_\indice{#5}}}

\newcommand{\myskew}[1]{\left[ #1 \right]^{\times}}

\renewcommand{\arraystretch}{1.5}

\newcommand{\sensor}[1]{\exposant{\text{{#1}}}}

\newcommand{\euler}{\operatorname{e}}
\newcommand{\unitmat}{\mathbb{1}}
